Raman spectroscopy of monolayer to bulk PtSe2 exfoliated crystals

Raman spectroscopy is widely used to assess the quality of 2D materials thin films. This report focuses on $\rm{PtSe_2}$, a noble transition metal dichalcogenide which has the remarkable property to transit from a semi-conductor to a semi-metal with increasing layer number. While polycrystalline $\rm{PtSe_2}$ can be grown with various crystalline qualities, getting insight into the monocrystalline intrinsic properties remains challenging. We report on the study of exfoliated 1 to 10 layers $\rm{PtSe_2}$ by Raman spectroscopy, featuring record linewidth. The clear Raman signatures allow layer-thickness identification and provides a reference metrics to assess crystal quality of grown films.

==> xx.tex <==




